Causal Inference using Gaussian Processes with Structured Latent Confounders

Latent confounders---unobserved variables that influence both treatment and outcome---can bias estimates of causal effects. In some cases, these confounders are shared across observations, e.g. all students taking a course are influenced by the course's difficulty in addition to any educational interventions they receive individually. This paper shows how to semiparametrically model latent confounders that have this structure and thereby improve estimates of causal effects. The key innovations are a hierarchical Bayesian model, Gaussian processes with structured latent confounders (GP-SLC), and a Monte Carlo inference algorithm for this model based on elliptical slice sampling. GP-SLC provides principled Bayesian uncertainty estimates of individual treatment effect with minimal assumptions about the functional forms relating confounders, covariates, treatment, and outcome. Finally, this paper shows GP-SLC is competitive with or more accurate than widely used causal inference techniques on three benchmark datasets, including the Infant Health and Development Program and a dataset showing the effect of changing temperatures on state-wide energy consumption across New England.

==> old.tex <==
% \section{Discussion}

% In Section~\ref{sec:Experiments}, we showed that GP-SLC produces accurate estimates of treatment effects in settings with hierarchical structure, despite latent confounding. While it not surprising that GP-SLC outperms the GP-NoConf and GP-NoObj baseline, its performance over the GP-PerObj baseline is striking. Intuitively, the GP-PerObj model can be defined as a GP-SLC model where the prior over the lengthscale of $U$ in $k_Y$ is a Dirac-delta function at $\infty$. In other words, if $U_i$ and $U_{i'}$ are not identical then $k_Y(Z_i, Z_{i'}) = 0$. As $U_i, U_i'$ are jointly Gaussian distributed, this occurs if and only if $i$ and $i'$ belong to the same object. This is not true of the GP-SLC model, which can place high posterior mass on $U_i$ being near $U_{i'}$ even if $i$ and $i'$ do not belong to the same object. In fact, the observed differences in performance can only be attributable to the GP-SLC model's ability to learn a latent representation $U$ that allows it to generalize across objects.

% The GP-SLC model we have presented assumes that data is observational, i.e. treatment assignment may be influenced by latent confounders and observed covariates. Modifying GP-SLC to model data drawn from randomized experiments is straightforward, we simply set the prior $P(\lambda_{UT}=\infty) = P(\lambda_{XT_{j=1...N_X}}=\infty) = 1$, removing any influence of $U$ or $X$ on $T$. 



% We use the slightly relaxed notation $T \sim Bernoulli(A)$ as shorthand for the function $f(A, \epsilon) = 1$ if $A > \epsilon$ and 0 otherwise, $\epsilon \sim uniform(0, 1)$.

%\footnote{Despite the fact that $(Y_*-Y)|T_*, T, Y, X, U, \Theta$ is Gaussian distributed, $ITE_{m=1...N_M}$ and thus $SATE_{T_*}$ are not due to the marginalization over $U,\Theta|X, T, Y$.}


% \vspace{-0.5cm}

%  We use bold notation to denote a vector or matrix. For matrices, such as $\X$, we use the corresponding row or column index to indicate a vector, e.g. $\X_i$ refers to the $m$'th instance's vector of covariates.


% To make predictions using a Gaussian process model, we first extend the joint distribution to include both observed targets $\Y$ and test targets $\Y_*$ as follows, where $\X_*$ is the set of corresponding test features.
% \vspace{-0.1cm}
% \begin{equation*}
%     P(\begin{bmatrix*}[l]\Y \\ \Y_*\end{bmatrix*}|\X, \X_*) \sim \mathcal{N}(\begin{bmatrix} 0 \\ 0 \end{bmatrix}, \begin{bmatrix*}[l]  \K(\X, \X) + \sigma^2 \textbf{I} & \K(\X, \X_*) \\ \K(\X_*, \X) & \K(\X_*, \X_*) \end{bmatrix*})
% \end{equation*}

% As the joint distribution over $\Y$ and $\Y_*$ is Gaussian, the conditional distribution $P(\Y_*|\Y, \X, \X_*)$ is also Gaussian distributed, with mean vector $\K(\X_*, \X) \inv{(\K(\X, \X) + \sigma^2 \textbf{I})}\Y$ and covariance $\K(\X_*, \X_*) - \K(\X_*, \X)\inv{(\K(\X, \X) + \sigma^2 \I)}\K(\X, \X_*))$. This formulation describes a Gaussian process model with additive Gaussian noise, where $\sigma^2$ is the noise variance.


%\footnote{Some controversy has emerged regarding adjustment for latent confounders in the multi-cause settings~\cite{d2019multi, ogburn2019comment, wang2019blessingscomment, Imai2019DiscussionOB}.}


% Causal graphical models (CGMs) provide a syntax and semantics for reasoning about interventions in a system of random variables. A CGM is defined as a tuple $G = (V, E)$ in which each vertex $v_i \in V$ represents a random variable and each edge $e_i \in E$ represents a local causal dependency. A CGM defines the structure of a functional causal model, a system of equations composed of a set of exogenous noise variables $\{\epsilon_1, ..., \epsilon_n\}$ and deterministic functions $\{f_1, ..., f_n\}$, one for each $v_i\in V$, in which the arguments to each function $f_i$ are the parents of $v_i$, or $Pa(v_i)$ in $G$. An intervention on a random variable $T$, denoted $do(T=t)$, operates on functional causal models by replacing the statement $T = f(Pa(T), \epsilon_T)$ with the deterministic statement $T=t$ before recomputing the assignment of all of $T$'s descendents. The interventional query $P(Y|do(T))$ differs from the conditional query $P(Y|T)$ in that intervening on $T$ does not modify the distribution of any of $T$'s ancestors in $G$.

% In practice, each $f$ is often unknown. Instead, one typically only has access to samples from the joint distribution $P(X_1, ..., X_n)$. Despite this limitation, it is often possible to infer the effects of an intervention, given appropriate assumptions about the causal graph structure. The do-calculus~\cite{Pearl2009Causality} provides a set of rules for translating an interventional query, i.e., the distribution of outcomes after intervening in the functional causal model, into an equivalent conditional query, which can be estimated from data alone. The simplest implication of the do-calculus is the back-door criterion, which states that $P(Y|do(T)) = \int P(Y|X, T)P(X) dX$, where $X$ is any subset of variables that block all d-connecting backdoor paths from $T$ to $Y$.

% It is common practice to assume that the latent functions in a structural causal model can be represented in simple parametric forms, such as the linear function with additive noise $f(T, \epsilon_T) = W \cdot pa(T) + \epsilon_T$. While these kinds of assumptions enable causal estimation in settings that would otherwise be unidentifiable \cite{Pearl2009Causality}, they often fail to capture complex relationships between random variables and thus may bias estimates of the effects of interventions. For example, patients' health may improve when exposed to small doses of a medication, while large doses can be harmful. In our work we relax these assumptions by assuming that the functions in a structural causal model are instead sampled from a Gaussian process prior.


% Figure~\ref{fig:CGM} shows GP-SLC as a causal graphical model, using plate notation to describe the shared confounding between instances. In the students scenario, $U$ represents unmeasured budgetary and political factors, $X$ represents all pre-treatment student-level covariates (e.g., household income), $T$ represents whether the student was held back, and $Y$ represents their future academic performance.

% Section~\ref{sec:GP-SLC} provides details on how GP-SLC induces a distribution over functional causal models, and how to produce fully Bayesian posterior estimates over counterfactual outcomes. In Section~\ref{sec:Theory} we show theoretically how these constraints enable consistent causal estimation and in Section~\ref{sec:Experiments} we show empirically how constraining latent confounders enables accurate counterfactual estimation in realistic hierarchical settings.



% \begin{table*}[h!]
%     \centering
%     \begin{tabular}{c|c|c}
%     \toprule
%     Dataset   & $f_t(X, U)$ & $f_y(X, T, U)$\\
%     \midrule
%     C L +     &  $X-U$ & $X+T+3U$\\
%     C L x     &  $(X+1)U$ & $(X+\frac{1}{10})TU$\\ 
%     C P +     &  $X-U^2$ & $X+\frac{1}{5}T^3+3U^2$\\  
%     C P x     &  $(X+\frac{1}{10})U^2$ & $\frac{1}{5}(X+\frac{1}{10})T^2U$\\  
%     C PS +     &  $X\text{sin}X - U\text{sin}U$ & $X\text{sin}X + T\text{sin}2T + 3U\text{sin}U$\\  
%     C PS x     &  $\frac{1}{10}(X\text{sin}X)(U\text{sin}U)$ & $\frac{1}{10}(X\text{sin}X)(T\text{sin}2T)(U\text{sin}U)$\\  
%     \bottomrule
%     \end{tabular}
%     \caption{The functional form of $T$ and $Y$ for 6 synthetic datasets with continuous treatments. The remaining 6 datasets share the identical functional form except $T$ is binarized.}
%     % \label{tab:mean_synthetic}
% \end{table*}{}


% \subsection{Gaussian Process Latent Variable Models}

% Unlike gaussian process regression models, in which the input features to each kernel function are observed, for gaussian process latent variable models the input to the kernel function is instead a latent variable with a known prior distribution $P(X)$. In other words, rather than computing the conditional distribution $P(Y_*|Y, X, X_*)$ as in the gaussian process regression case, we instead seek to compute $P(X|Y) = \frac{P(Y|X)P(X)}{\int P(Y|X)P(X) dX}$ and related conditional distributions such as $P(Y_*| Y)$. However, these conditional distributions are generally intractable due to nonlinearities in the data marginal. Several approximate techniques exist for addressing this intractability, including MAP optimization (cite original GPLVM paper), variational inference (cite bayesian GPLVM paper), and sampling-based methods (find papers).


% \section{Mapping to Standard Causal Designs}

% The generative model we have described in section \ref{sec:GPROC} described a general template for causal inference when latent confounders are not i.i.d, and are instead related by background knowledge about shared objects across samples. In this section we discuss how bayesian nonparametric versions of several standard causal designs can be expressed using this template.

% \subsection{Within Subjects Randomized Experiment}

% TODO: Expand on below text.

% Setting the covariance kernel of $k_T$ to be $\delta_{i,j} * \sigma_T$ is equivalent to a randomized treatment assignment, i.e. data where the treatment is independent of the latent confounder.

% \subsection{Longitudinal Studies}

% Longitudinal studies follow sets of individuals over extended periods of time, and often involve the repeated measurement of several random variables.

% TODO.

% \subsection{Interrupted Time-Series Designs}

% TODO.

% \subsection{Twin Studies}

% TODO.

% \section{Common Causal Estimands}

% TODO: Describe how standard causal estimands can be expressed as functionals of interventional outcomes like $Y_t$. We may need to add additional terms if we want to follow things like ATE strictly, which are defined as the \textit{difference} between distinct interventional outcomes. This will become a bit challenging with continuous treatment variables, but not impossible.

% We assume continous treatment throughout the study but the exntention to discreate treatment is simple. We are interested in identifing the mean of interventional distribution (dose-response curve), $\mathrm{E}[Y(T=t)] = \mathrm{E}[Y|do(T=t)]$. In discussion section, or appendix, we mention that any causal estimand in the form of $g(P[Y|do(T=t1)]) - g(P[Y|do(T=t2)])$ can be also identified, which is a contrast between the marginal complete interventional distributions. This includes ATE, SATE, CATE, and possibly more such as risk ratio.

% \subsection{Average Treatment Effect}

% TODO.
% the population-level average treatment effect 
% \begin{gather}
%     \nonumber \tau_{ATE} = \mathrm{E}[Y_{t=1} - Y_{t=0}]\\ = \mathrm{E}[P(Y | do(T=1)) - P(Y | do(T=0))]
% \end{gather}{}
% \subsection{Sample Average Treatment Effect}
% TODO.
% the finite-sample average treatment effect 
% \begin{gather}
%     \tau_{SATE} = \frac{1}{N} \sum^N_{i=1}[Y_{t=1,i} - Y_{t=0,i}]\\
%     = \frac{1}{N} \sum^N_{i=1}[P(Y_i | do(T_i=1)) - P(Y_i | do(T_i=0))]
% \end{gather}{}

% \subsection{Conditional Average Treatment Effect}
% TODO.

% \subsection{Object Conditional Average Treatment Effect}
% Object Conditional Average Treatment Effect (OCATE) for an object $\mathcal{O}$ is 
% \begin{gather}
%     \tau_{OCATE} = \frac{1}{|\mathcal{O}|} \sum_{j=1}^{|\mathcal{O}|}[Y_{t=1,j} - Y_{t=0,j}] \\
%      = \frac{1}{|\mathcal{O}|} \sum_{j=1}^{|\mathcal{O}|}[P(Y_j | do(T_j=1)) - P(Y_j | do(T_j=0))]
% \end{gather}{}

% TODO.


% \subsection{Section header TBD}

% As $P(U, T, Y|\alpha, \beta, \gamma, \sigma_U^2, \sigma_T^2, \sigma_Y^2)$ is jointly gaussian, the marginal distribution over observed variables $P(T, Y|\alpha, \beta, \gamma, \sigma_U^2, \sigma_T^2, \sigma_Y^2)$ is also jointly gaussian. Without loss of generality, we have the following.

% \begin{gather}
% \nonumber    P(T, Y|\alpha, \beta, \gamma, \sigma_U^2, \sigma_T^2, \sigma_Y^2) \sim \mathcal{N}(0, \begin{bmatrix}
% \Sigma_{TT} & \Sigma_{TY} \\
% \Sigma_{YT} & \Sigma_{YY}
% \end{bmatrix})
% \end{gather}{}

% The covariance matrix of $T$ and $Y$ can be equivalently expressed in terms of \textit{observed variable} $\Sigma_U$ and \textit{latent variables} $\sigma_U^2, \sigma_T^2, \sigma_Y^2, \alpha, \beta$ and$, \gamma$ via the following.

% \begin{equation}
%     \begin{gathered}
%     \Sigma_{TT} = \alpha^2\sigma_U^2 \Sigma_U + \text{diag}(\sigma_T^2)\\
%     \Sigma_{TY} = \alpha(\beta\alpha + \gamma) \sigma_U^2\Sigma_U + \gamma \text{diag}(1)\\
%     \Sigma_{YY} = (\beta\alpha+\gamma)^2 \sigma_U^2\Sigma_U + (\beta^2+1) \text{diag}(\sigma_Y) \label{eq:lin3}
%     \end{gathered}
% \end{equation}{}


% \begin{proof}
% The system of linear equations (\ref{eq:lin3}) has 3N equations and N+3 unknown parameters. By additional assumptions of block diagonal, $\Sigma_U$ is parameterized by the number of blocks $M$. Since all off-diagonal blocks in $\Sigma_U$ are 0, (\ref{eq:lin3}) can be decomposed into $M$ system of equations, one for each block. For $i$th block in $M$ with size $m_i \times m_i$, there and 3$m_i$ equations and 4 unknown parameters. Thus (\ref{eq:lin3}) has a unique solution if $m_i > 1$ for all $i \in [1 \dots M]$, and $\gamma$ is identifiable.
% \end{proof}
% The theorem above materializes object conditioning in the prior of $\Sigma_U$. Specifically, the block $M$ represents each object and size of $M$ represents the membership of the object. Given this theorem, standard M-estimation such as maximum likelihood estimation gives asymptotically consistant estimate of $\gamma$, and subsequently, the unbiased estimate of $\mathbf{E}[Yt]$ by substituting $\gamma$ with $\hat{\gamma}$ in (\ref{eq:lin_intervention}).

% \subsection{Identifiability and Convergence}

% TODO. We'll need to be very careful about what we mean by identifiability here, as we're out of graphical models land. One stringent definition could be that the prior and the posterior are identical given any data. Another more lenient definition could be that even with infinite data the posterior variance doesn't collapse to 0. The difference between these two is that for the second, data may update our beliefs, but it might not ever get to the truth. I've described the theorems below in terms of the more lenient definition.

% \textbf{Definition 1: Identifiability.} A causal query is identifiable for a GPROC model if and only if it converges in probability to a dirac-delta function as the number of data instances approaches infinity.

% \textbf{Theorem 1: GPROC identifies the mean over interventional distribution $\mathbf{E}(Y(a))$ if we assume the covariance matrix for confounding $\Sigma_U$ is a positive diagonal matrix.} \\
% Sketch: \\
% GPROC models the output distribution $P(Y_t|U, \lambda, T, Y, X)$ via Gaussian Process. We are going to show that the mean of interventional distribution is identifiable from observational data by marginalizing over $U$ if $U$ satisfies uncounfoundedness and positivity. (Argument from backdoor criterion, g-formula, adjustment)\\\\
% Proof: 
% \begin{enumerate}
%     \item Positivity $1 > P(T=t|X, U) > 0$ is satisfied by GPROC for continuous treatment t from modeling assumption.
%     \item Uncounfoundedness is satisfied when $\Sigma_U$ is a positive diagonal matrix. By the construction of the covariance kernel, confounding for each data instance ($i \neq j$) is independent. Also for the fixed data instance indexed by $i$, $u_i$ is drawn iid from $\mathcal{N}(\mu_{ui}, \sigma_{ui})$. Treatment variable $T_i$ is a function of $u_i$ (and exogenous noise?). Since each instance of $T_i$ is computed as a function of iid random variable, $T_i$ is also iid random variable (formally by measure theory)
%     % \item Use 
% \end{enumerate}{}
% GP renders the distribution over function. this is analogous to di finetti theorem which states that exchangeability implies there exists a latent variable that renders variables iid. In our case such latent variable is the function we apply during inference. 

% comment RCT or meta-RCT identifies causal effect
% 1. When U is drawn iid (constant mu, constant times identity matrix) then GPROC simulates RCT
% 2. When U is drawn independently (off diagonal being zeros), then GPROC simulates meta RCT


% \textbf{Theorem 2: Identifiability with no Object Conditioning.} If $k_T \neq \delta_{i,j} \sigma_T$ for some constant $\sigma_T$ and $\Sigma_{U,i,j}=0$ for all $i \neq j$, ATE, SATE, CATE, and OCATE are not  identifiable.
% 0) $P(Y_t|...U)$ depends on U
% 1) P(U|T,Y) does not converge -> is there a way to show?
% if U is not deterministic, the only case where $P(Y_t|...U)$ does not depend on U is when U is constact within the object (but unknown value)

% example: two individual, different X, similar $Y_t$
% 1, either u's are close (probability of two indeviduals belong to the same object)
% or 2, length scale X is large for X (allowing uncertainty for X within the same object)


% \textbf{Theorem 3: Identifiability of Within Subjects Observational Studies - With Object Conditioning. - All instances same object} If $k_T \neq \delta_{i,j} \sigma_T$ for some constant $\sigma_T$ and there exists a $j$ such that $\Sigma_{U,i,j}=1$ for all $i$, ATE, SATE, CATE, and OCATE are identifiable.\\\\


% \textbf{Theorem 4: Identifiability of Within Subjects Observational Studies - With Object Conditioning. - 2 instances each, infinite objects.}

% sketch:\\
% By linearity of expectation, we can decompose target causal estimand as a convex sum of causal estimands from each object. Show 1) all causal estimands above are identifiable with object conditioning given $u_i$ = $u_j$  i and j belong to the same object. 2) each object is sampled iid from population, meaning $\mathbf{E}[\frac{\sum_i^N\mathrm{I}\{x_i \in \mathcal{O}\}}{|\mathcal{O}|}] \xrightarrow{}  P(\mathcal{O})$. Then all causal esitmands above are identifiable and unbiased in expectation.

% \subsection{Finite Sample Posterior Variance}

% \textbf{Theorem 4: Posterior Variance of Object Conditioned Randomized Experiments.} If $k_T = \delta_{i,j} \sigma_T$ for some constant $\sigma_T$, ATE, SATE, CATE, and OCATE all have lower posterior variance for any finite dataset when some off-diagonal elements of $\Sigma_U$ are non-zero.

% \textbf{Theorem 5: Posterior Variance of Object Conditioned Observational Studies.} If $k_T \neq \delta_{i,j} \sigma_T$ for some constant $\sigma_T$, ATE, SATE, CATE, and OCATE all have lower posterior variance for any finite dataset when some off-diagonal elements of $\Sigma_U$ are non-zero.


% We define the GPROC structural model as follows, which is parameterized by exogenous noise, $\epsilon_X$, $\epsilon_T$, and $\epsilon_Y$, kernels $k_X$, $k_T$, and $k_Y$, latent scaling factor $\sigma_U$, and block-diagonal object conditioning matrix $\Sigma_U$. In our experiments in Section~\ref{sec:Experiments} we assume that $\Sigma_U$ is known, exogenous noise is sampled from independent gaussians, and that structural functions are generated from RBF kernels with automatic relevance determination. We place priors over exogenous noise variance, latent scaling factor $\sigma_U$, and kernel hyperparameters.\footnote{The expression $[U_{1, j}, ..., U_{n, j}] \sim N \mathcal(0, \Sigma_U\sigma^2_{U_j})$ is shorthand for generating exogenous $\epsilon_i \sim \mathcal{N}(0, 1)$ and then defining $f_U$ as a $A \cdot [\epsilon_{1, j}, ..., \epsilon_{n, j}]$, where $A \cdot A^T$ is the cholesky decomposition of $\Sigma_U\sigma^2_{U_j}$.} Here $i$ indexes the data instance (units), $j$ indexes the dimension of the latent confounders, and $l$ indexes the dimension of the observed confounders.
% \vspace{-0.1cm}
% \begin{equation*}
%         \begin{bmatrix}U_{1, j}, ..., U_{n, j}\end{bmatrix} \sim N\mathcal(0, \Sigma_U \sigma^2_{U_j}) \quad \quad \quad
% \end{equation*}
% \vspace{-0.50cm}
% \begin{equation}
%     \begin{aligned}
%         f_X &\sim GP(0, k_X)\\
%         f_T &\sim GP(0, k_T) \\
%         f_Y &\sim GP(0, k_Y)
%     \end{aligned}
%     \quad
%     \begin{aligned}
%         X_{i, l} &= f_X(U_i, \epsilon_{X_{i, l}})\\
%         T_i &= f_T(U_i, X_i, \epsilon_{T_i})\\
%         Y_i &= f_Y(U_i, X_i, T_i, \epsilon_{Y_i})
%     \end{aligned}
%     \label{eq:GPROC}
% \end{equation}

%  and that background knowledge of hierarchical structure constrains the distribution over latent confounders $U$. We represent this background knowledge in the covariance matrix $\Sigma_U$, which encodes joint structure amongst individuals' latent confounding variables. For example, if we know that the $i$ and $i'$th samples belong to the same object and we assume that their latent confounders are identical, i.e., $P((U_i = U_i') = 1)$, then we set $\Sigma_{U,i,i'} = \Sigma_{U,i',i} = 1$. If we instead expect the $i$ and $i'$th samples to have similar but not identical latent confounders, we would instead assign $0 < \Sigma_{U,i,i'} = \Sigma_{U,i',i} < 1$. $\sigma_U^2$ can be thought of as a (latent) scaling factor for unobserved confounding.

% \subsection{Priors over GPROC functional models}

        
        
        % \begin{align*}
        %         k_{X_{j=1...N_X}}(U_o, U_{o'}) &= \sigma_{X_j} \exp{(-\sum_i^{N_U} \frac{\left\|U_{o,i} - U_{o',i}\right\|^2}{\lambda_{UX_{i, j}}})}\\
        %         k_{T}([U_o, X_{m}], [U_{o'}, X_{m'}]) &= \sigma_{T} \exp{(\sum_i^{N_U} \frac{\left\|U_{o, i} - U_{o',i}\right\|^2}{\lambda_{UT_i}} + \sum_j^{N_X} \frac{\left\|X_{m, j} - X_{m', j}\right\|^2}{\lambda_{XT_{j}}})}\\
        %         k_{Y}([U_o, X_{m}, T_{m}], [U_{o'}, X_{m'}, T_{m'}]) &= \sigma_{Y} \exp{(\sum_i^{N_U} \frac{\left\|U_{o, i} - U_{o',i}\right\|^2}{\lambda_{UY_i}} + \sum_j^{N_X} \frac{\left\|X_{m, j} - X_{m', j}\right\|^2}{\lambda_{XY_{j}}} + \frac{\left\|T_m - T_m'\right\|^2}{\lambda_{TY}})}
        % \end{align*}
        
        
        
% \subsection{Robustness to Collider Bias}
% \label{subsec:collider}

% Thusfar we have demonstrated that when underlying structural assumptions are satisfied, i.e., members of the same object hierarchy share latent confounders, GP-SLC produces accurate estimates of individual and population-level counterfactual outcomes. However, such assumptions are likely to be violated in real settings. One example violation could be that parent objects don't share confounding variables, but instead share common effects of treatment and outcome variables. It is well known that \textit{conditioning} on an observed collider introduces bias into causal estimates~\cite{berkson1946limitations}. However, recent work has demonstrated that conditioning on objects does not introduce such biases~\cite{jensen2019object}. In the student retention example we introduced in Section~\ref{sec:Introduction}, such a common effect could be the proportion of students who later attend a post-graduate degree. In practice, collider bias is mitigated by conditioning on only pre-treatment variables \cite{montgomery2018conditioning}, however conditioning on pre-treatment variables can sometimes introduce similar baises, a phenomenon known as m-bias~\cite{liu2012implications}.

% To test GP-SLC's performance in the presence of such common effects (colliders), we generate synthetic data in which each $T_i$ and $Y_i$ are sampled independently from a $\mathcal{N}(0,1)$ distribution. We then randomly partition the dataset into pairs $i, i'$ and assign colliders $U_i = U_{i'} = T_i + T_{i'} + Y_i + Y{i'}$. Figure~\ref{fig:collider} shows the results the GP-SLC model's counterfactual estimates compared against two OLS baselines, one that incorrectly assumes $U$ is a confounder (OLS w/ Collider) and one that regresses only on $T$ (OLS w/out Collider). While the GP-SLC model achieves worse counterfactual predictions than the OLS model regressed only on T, this is likely a result of using a higher capacity regression model and not due to collider bias. When the posterior samples of $U$ are omitted from the counterfactual estimation procedure (GP-SLC w/out U), the estimated average counterfactual outcomes only minimally change.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/collider.png}
%     \caption{Results of the GP-SLC model applied to a synthetic dataset where $U$ is a collider of all $T$ and $Y$ belonging to the same object. Unlike the OLS baseline that incorrectly assumes $U$ is a confounder, GP-SLC is robust to structural misspecification. The value of the collider is indicated by the color of the data points.}
%     \label{fig:collider}
% \end{figure}

% We examine the finite-sample behavior of the GP-SLC model with a diversity of synthetic datasets. We consider the scenario under the existance of \textit{object-level} latent confounders ($U$) that simultaneously influence observed treatment ($T$), covariates ($X$), and outcomes ($Y$). The general process is as follows. First, we generate $N_O$ variables $U \in \mathbb{R}^3$ from a multivariate normal distribution $\mathcal{N}(\mu_U, \Sigma_U)$ where $\mu_U=(0,0,0)^T$ and $\Sigma_U = 0.5I$. Then we define additional covariates $X \in \mathbb{R}^3$ given $U$ as $x_i \sim \mathcal{N}(Wu_i^T, 0.5I)$ where $W$ is a 3x3 weight matrix from a multivariate normal distributon with mean $(0,0,0)^T$ and an identity covariance matrix.

% In order to generate treatment $T$ given $X$ and $U$, we first define functions $f_t := \mathbb{R}^3 \xrightarrow{} \mathbb{R}$ and $g_t := \mathbb{R}^3 \xrightarrow{} \mathbb{R}$. Then we generate a treatment for the $i$th unit from normal distribution whose mean is the sum of $f_t(x_i)$ and $g_t(u_i)$ i.e., $t_i \sim \mathcal{N}(f_t(x_i)+g_t(u_i), 0.5)$. We also repeat the experiment with a product i.e., $t_i \sim \mathcal{N}(f_t(x_i)g_t(u_i), 0.5)$. While this method generates a continous $T$, we can easily binarize it by replacing $t_i$ with $\text{Bernoulli}(\text{expit}(t_i))$. Simimlarly, we generate an outcome variable $Y$ given $X$, $U$ and $T$ with an additional function $h_y := \mathbb{R} \xrightarrow{} \mathbb{R}$ i.e., $y_i \sim \mathcal{N}(f_y(x_i)+g_y(u_i)+h_y(t_i), 0.5)$ or $y_i \sim \mathcal{N}(f_y(x_i)g_y(u_i)h_y(t_i), 0.5)$. 

% Our synthetic data is configured by a tuple of three items; treatment assignment, functinoal form, and interaction. Treatment assignment takes either C (continuous) or B (Binary), which determines if we binarize an otherwise continous $T$. Functional form takes one of L (Linear), P (Polynomial), PS (Polynomial x Sinusoidal), which determines the local functional dependency of $X$, $U$ and $T$. Finally, interaction takes either + (additive) or x (multiplicative), which determines how we aggregate f(X), g(U), and h(T). We summarize the mean of $T$ and $Y$ for 6 synthetic datasets with continuous $T$ in Table \ref{tab:mean_synthetic}. Also, we define 6 additional datasets by binarizing $T$. For each of 12 configurations, we generate 200 data instances from 20 objects of equal size. 

% \begin{table*}[htbp]
% \setlength\tabcolsep{4pt}
% \label{tab:synthetic}
%   \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc}
%     \toprule
%     \multirow{2}{*}{Dataset}  &
%       \multicolumn{2}{c}{\textbf{GP-SLC}} &
%       \multicolumn{2}{c}{GP-NoConf} &
%       \multicolumn{2}{c}{GP-NoObj} &
%       \multicolumn{2}{c}{GP-PerObj} & \multicolumn{2}{c}{MLM1} & 
%       \multicolumn{2}{c}{MLM2} &
%       \multicolumn{2}{c}{BART}\\
%       & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} \\
%       \midrule
%         C L + & 0.42 & 0.21 & 46.78 & 30.49 & 44.35 & 28.26 & 10.08 &3.30 &1.00 &0.31 &\textbf{0.40} & \textbf{0.11}& 16.17 & 7.68 \\
%         B L + & \textbf{0.04} & \textbf{0.00} & 9.33 & 8.76 & 9.32& 8.71& 2.91& 0.60& 0.38& 0.04 & 0.23& 0.01 & 1.26 & 0.06 \\
%         C L x & 13.91 &9.36 & 10.53 & 4.25 & 11.50 &5.85 & 3.56 & 0.13 &18.01 &\textbf{0.87} &\textbf{9.42} & 1.84 & 14.89 & 9.16 \\
%         B L x & 1.19 &\textbf{0.02}  &1.75  &0.15  & 1.67 &0.15 & \textbf{1.10}& 0.05 &1.86 &0.10 &  1.78& 0.08& 1.62 & 0.04\\
%         C P + & 2.53 & 1.65& 29.97& 18.34& & & 8.84 &2.82 & 5.34 &2.45 &2.17 &1.39 & 16.14 & 10.60 \\
%         B P + & \textbf{0.02}& \textbf{0.00} & 3.14 &2.60 &2.70 & 1.83 & 8.24 &2.68 & 0.35 &\textbf{0.00} &0.23 & \textbf{0.00}& 0.64 & 0.02 \\
%         C P x & 2.68 & 2.20 &  &  & & & & & & & & & 9.53 & 7.89 \\
%         B P x &  &  & & &  & & & & & & & & 0.15 & 0.00 \\
%         C PS + &  &  &  & &  & & & & & & & & 77.42 &57.14 \\
%         B PS + & &  &  & &  & &  & &  & & & & 1.28 & 0.74 \\
%         C PS x & & & & && &  & & & & & & 23.51 & 12.46 \\
%         B PS x &  & & & && &  & &  & & & & 20.37 & 9.97  \\
%     \bottomrule
%   \end{tabular}
%   \caption{Results of the GP-SLC model and various baselines on 12 synthetic datasets. We vary treatment assignment (Continuous - C and Binary - B), functional form, (Linear - L, Polynomial - P, and a Sinusoid x Polynomial - PS), and interactions ($f(T,X,U) = f(T) + f(X) + f(U)$ and $f(T,X,U) = f(T)f(X)f(U)$). Lower is better.}
% \end{table*}


% \begin{table*}[htbp]
% \setlength\tabcolsep{4pt}
% \label{tab:synthetic}
%   \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc}
%     \toprule
%     \multirow{2}{*}{Dataset}  &
%       \multicolumn{2}{c}{\textbf{GP-SLC}} &
%       \multicolumn{2}{c}{GP-NoConf} &
%       \multicolumn{2}{c}{GP-NoObj} &
%       \multicolumn{2}{c}{GP-PerObj} & \multicolumn{2}{c}{MLM1} & 
%       \multicolumn{2}{c}{MLM2} &
%       \multicolumn{2}{c}{BART}\\
%       & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} & {PEHE} & {MSE} \\
%       \midrule
%         C PS + & \textbf{9.10} & \textbf{5.33} & 194.12 &134.91 & 202.15 &143.65 & 33.83& 18.07 &10.64 & 5.47& 12.26& 8.50& 77.42 &57.14 \\
%         % B PS + & \textbf{0.68} & 0.51 & 39.64 & 12.13& 44.07 & 9.67 & 33.17 &12.73 & 2.91 & 0.73& 1.73& \textbf{0.27} & 1.28 & 0.74 \\
%         C PS x & \textbf{8.98} &2.92 & 37.57&22.30 &40.52& 23.52& 10.07 & \textbf{2.68} &21.21 &8.38 &39.08 & 27.04 & 23.51 & 12.46 \\
%         % B PS x & 73.27 & 22.09&29.93 & 9.67 & 61.70& 18.16 &  & &66.84 &20.53 & 55.67 & 14.60 & 20.37 & 9.97  \\
%     \bottomrule
%   \end{tabular}
%   \caption{Results of the GP-SLC model and various baselines on 12 synthetic datasets. We vary treatment assignment (Continuous - C and Binary - B), functional form, (Linear - L, Polynomial - P, and a Sinusoid x Polynomial - PS), and interactions ($f(T,X,U) = f(T) + f(X) + f(U)$ and $f(T,X,U) = f(T)f(X)f(U)$). Lower is better.}
% \end{table*}




% We can define ground-truth individual treatment effect given the intervention $do(T = T_*)$ as follows:
% \begin{equation}
%     \begin{aligned}
%         ITE_{T_*, m} = f_y(X_m, T_*, U_{o=pa(m)}) - f_y(X_m, T_m, U_{o=pa(m)})\\
%         SATE_{T_*} = \frac{1}{N_M}\sum_{m=1}^N ITE_{T_*, m}
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         \text{SATE error} = \mathbb{E}_{t \in \text{doT}}[(\mathbb{E}_{m \in M} [Y^*_{t, m}] - \mathbb{E}_{m \in M} [\hat{Y}_{t, m}])^2]\\
%         \text{ITE PEHE} = \mathbb{E}_{t \in \text{doT}}\underbrace{\mathbb{E}_{m \in M}[(Y^*_{t, m} - \hat{Y}_{t, m})^2]}_\text{$PEHE_t$}
%     \end{aligned}
% \end{equation}

% For each synthetic data, we binarize the treatment $T$ in equations~\ref{eq:synthetic_structural} by applying 
% \begin{equation}
%     \begin{aligned}
%         T_{\text{bin}_i} \sim \text{Bernoulli}(1/1+\text{exp}(-T_i)) 
%     \end{aligned}
% \end{equation}

% In total, we 

% We define 6 pairs of functions for $f_t$ and $f_y$ in Table \ref{tab:mean_synthetic}. 


    % C L +     &  $X-U$ & $X+T+3U$\\
    % C L x     &  $(X+1)U$ & $(X+\frac{1}{10})TU$\\ 
    % C P +     &  $X-U^2$ & $X+\frac{1}{5}T^3+3U^2$\\  
    % C P x     &  $(X+\frac{1}{10})U^2$ & $\frac{1}{5}(X+\frac{1}{10})T^2U$\\  
